Muon Capture on the Deuteron -- The MuSun Experiment

We propose to measure the rate \Rd\ for muon capture on the deuteron to better than 1.5% precision. This process is the simplest weak interaction process on a nucleus that can both be calculated and measured to a high degree of precision. The measurement will provide a benchmark result, far more precise than any current experimental information on weak interaction processes in the two-nucleon system. Moreover, it can impact our understanding of fundamental reactions of astrophysical interest, like solar pp fusion and the $\nu+d$ reactions observed by the Sudbury Neutrino Observatory. Recent effective field theory calculations have demonstrated, that all these reactions are related by one axial two-body current term, parameterized by a single low-energy constant. Muon capture on the deuteron is a clean and accurate way to determine this constant. Once it is known, the above mentioned astrophysical, as well as other important two-nucleon reactions, will be determined in a model independent way at the same precision as the measured muon capture reaction.

==> BeamRequest.tex <==
\section{First Beam Request}


==> MuonCapture.tex <==
\section{Muon Capture on the Deuteron}
\label{MuonCapture}
              
\subsection{Theory}
The $\mu d$ reaction provides a necessary stepping stone in connecting 
the muon capture on a single nucleon ($\mu p$) to capture on heavier nuclei, 
e.g., $^3$He and $^4$He~\cite{Gorringe:2002xx}.
The natural theoretical frame work to make this transition is EFT, especially 
chiral perturbation theory (ChPT).
It inherits the relevant symmetries of QCD and the  
parameters in ChPT are linked to matrix elements of QCD operators. 
It is very successful in describing observables in the one nucleon sector. 
This theory has thus been applied to, e.g., $\mu p$ capture.
As we will see, it can also be (and has been) applied to two-nucleon systems, 
like $\mu d$ capture, and can be extended to $\mu$ capture on heavier nuclei, 
e.g., $\mu^3$He capture reactions. 

EFT offers a valuable theoretical framework for 
sufficiently low energy-momentum regimes. 
As noted by Weinberg~\cite{Weinberg:1990rz,Weinberg:1991um,Weinberg:1992yk}, 
one can construct an effective field theory (EFT) applicable to 
multi-nucleon systems. 
EFT relies on an expansion scheme where the 
small parameter is $Q/\Lambda \ll 1$ where $Q$ is the 
four-momentum of the relevant process. 
The expansion is in powers $(Q/\Lambda)^\nu$ where the 
higher order terms give smaller corrections to the 
dominant lowest order terms. 
The {\it effective} nature of EFT is reflected 
in the presence of unknown coefficients, 
called the low-energy-constants (LECs), 
which parameterize the high-energy physics 
that has been integrated out in generating the low-energy EFT. 
In principle these LECs can be evaluated from QCD 
but in practice they are determined from experimental data. 
Once the LECs are determined the theory 
will make unambiguous predictions of observables for 
many different processes. 
For example, the $\mu p$ capture rate has been 
evaluated including one-loop corrections, 
a level of precision  that include several LECs that are 
determined empirically from other reactions~\cite{Ando:2000zw}. 
The pseudo-scalar constant $g_P$, linked to the pion pole contribution in 
$\mu p$ capture, is evaluated to 
two-loops precision in ChPT and gives a unique expression for $g_P$ in terms 
of the fundamental LECs, $f_\pi$ and $g_A$, which are assumed known.  
 
In the pion-less EFT (where the pion is considered a high-energy degree 
of freedom) the expansion parameter is $ Q/m_\pi\ll1$, where $Q$ is a typical 
energy or momentum of the reaction and $m_\pi$ is the pion mass.
In ChPT, on the other hand, the expansion parameter is $ Q / \Lambda_\chi\ll1$,
where $\Lambda_\chi \simeq 4\pi f_\pi \simeq m_N $ with $m_N$ the nucleon mass.
At very low energies ($Q\ll m_\pi$) the pion-less EFT is very useful. 
However, for $\mu d$ capture $Q \simeq m_\pi$, ChPT, which is valid 
over a much larger energy-momentum region, is a better theory. 
This conclusion is also obvious from Fig.~\ref{dp}, which show the entire phase 
space available for the $\mu^-d\to\nu_\mu nn$ reaction.
The pion-less EFT applies only in the bottom left part of the figure, as indicated.
In contrast, ChPT is valid for the entire phase space, with some modifications perhaps
needed in the region closer to the $p_\nu=0$ point, the so-called ``dangerous 
region''~\cite{Ando:2001es}, where the momentum transfer becomes large.
However, as shown in that paper, the contribution from this region to the 
total capture rate is marginal.
The larger range of allowed energies also allows ChPT to be applied to more 
processes than pion-less EFT.

At the desired level of precision the two-nucleon system has one new unknown 
LEC characterizing the short-distance two-nucleon axial current. 
This LEC is called $L_{1A}$ in pion-less theory~\cite{Chen:2005ak} and 
$\hat{d}^R$ in ChPT~\cite{Ando:2001es}.
In the latter case the pion-exchange currents between the two nucleons 
are explicitly evaluated, while they are embedded in 
$L_{1A}$ in the pion-less EFT. 
The coupling constant $\hat{d}^R$ enters in a range of important weak
and pionic reactions, i.e., $\mu d$, $pp$ fusion~\cite{Park:2002yp}, $\nu d$ 
reactions~\cite{Nakamura:2002he}, and 
pion radiative capture on the deuteron~\cite{Gardestig:2006hj}. 
At present, $\hat{d}^R$ is determined from triton beta decay but theoretically 
it is highly desirable to determine its value within the two-nucleon system. 
Once $\hat{d}^R$ is determined in this way, the solar $pp$ fusion and 
$\nu d$ SNO reactions will be determined in a model independent way 
at the same precision as the measured $\mu d$ capture reaction.
Recent developments have also made it possible to derive the deuteron and 
scattering state wave functions within chiral perturbation 
theory~\cite{Phillips:1999am,Gardestig:2005pp,Kaiser:1997mw,Epelbaum:1999dj,
Rentmeester:1999vw,Entem:2003ft}, without having to resort to the hybrid 
approach of using phenomenological wave functions.
Thus all the relevant two-nucleon processes can be calculated entirely within
the same consistent framework.
The solar $pp$ fusion reaction is presently theoretically 
calculated at an estimated 2--3\% level~\cite{Adelberger:1998qm}. 
One strives to achieve a more accurate rate for this primary solar fusion 
process which is one of the key inputs that controls the solar model.  
A more refined understanding of the solar model is wanted since this 
model is often used as a testing ground for computer simulation 
of the burning of stars.
The theoretically evaluated low energy solar neutrino reactions, 
$\nu_e + d \to  e + p + p$ and 
$\nu_l + d \to \nu_l + p + n$ are used to analyze the SNO data. 
A high precision evaluation of the charged- and neutral-current reaction 
cross sections will allow a more precise determination of 
neutrino oscillation parameters from the SNO data. 
Furthermore, studying few-nucleon systems also helps us to improve 
our understanding of electroweak phenomena in more 
complex nuclei, which feature in a wide variety 
of astrophysical phenomena including neutrino-nucleosynthesis. 

As already mentioned, the LEC $\hat{d}^R$ also connects $\mu d$ to 
$\pi^-d \to\gamma nn$. 
This radiative pion capture process is considered to be the currently most 
reliable (experimentally and theoretically) method of extracting the $nn$ 
scattering length ($a_{nn}$)~\cite{Machleidt:2001rw}, while the alternative 
method of using the three-nucleon process $nd\to nnp$ is plagued with 
inconsistent results~\cite{GonzalezTrotter:2006wz,Huhn:2001yk}.
The difference of the $nn$ and $pp$ scattering lengths is used to constrain the
charge-symmetry-breaking pieces of the modern high-precision phenomenological
nucleon-nucleon potentials, which in turn are needed for detailed understanding
of the lighter nuclei ($A<20$, say)~\cite{Wiringa:1994wb,Pieper:2001mp}.
The theoretical error in $a_{nn}$ extracted from $\pi^- d\to\gamma nn$ can 
with ChPT methods be reduced to $\pm0.05$~fm, i.e., to the 
0.3\% level~\cite{Gardestig:2005pp,Gardestig:2006hj,Gardestig:2006jd}.
However, this precision can be reached only if the short-range physics is 
constrained by $\hat{d}^R$.
Thus a precision measurement of $\mu d$ would also help in establishing a 
precise value of $a_{nn}$ completely within the two-body sector and ChPT.

At the level of precision aimed at in the proposed $\mu d$ 
capture experiment, an evaluation of 
the radiative corrections will be necessary. 
Traditionally, the evaluation of radiative 
corrections for a nucleon is based on either the quark picture 
or the pre-EFT hadronic picture. 
In the former, the calculation is well defined
at the quark-lepton level~\cite{Marciano:1985pd},
but it is not easy to assess theoretical uncertainties
that might creep in as the amplitudes for the current quarks are translated 
into those for the physical hadrons. 
Meanwhile, calculations based on the pre-EFT hadron picture
involve intrinsic model dependence, since it is not equipped 
with a systematic method of describing short-distance physics.
In contrast, ChPT provides a reliable systematic framework
which respects all required symmetry properties
and wherein one can enumerate and evaluate
all the relevant Feynman diagrams up to a specified
chiral order (see, e.g., \cite{Bernard:1995dp}).
The ChPT evaluation of radiative corrections of neutron $\beta$-decay was 
developed in Ref.~\cite{Ando:2004rk},  and this formalism can be readily 
applied to $\mu p$ capture.
This treatment involves unknown LECs associated with photon loops,
which need to be determined empirically. 
Once these LEC are constrained using the high-precision
data on neutron $\beta$-decay and $\mu^-p$ capture we can 
apply them in the calculations of the $\mu d$ radiative corrections.
No new LECs are thus needed for the radiative corrections to $\mu d$.


The final 3-body state covers a broad range of momentum transfer to the 
2-N system (see~Fig.\ref{dp}). 
In adequate non-relativistic kinematics the total energy $Q= 102.1~MeV$ in the 
final state is the sum of the neutron CMS energy, two neutron relative energy 
$E_{nn}$, and the neutrino momentum $p_\nu$.
\begin{equation}
Q= \frac{p_\nu^2}{4 M_n} + E_{nn} + p_\nu
\end{equation}
Thus the kinematics can be parametrized either by $E_{nn}$ or equivalently by   $p_\nu$.
The properties of the 2-N system enter, in particular the deuteron wave function 
in the initial and the neutron scattering length $a_{nn}$ in the final state. 
Furthermore, two-body currents contribute, making process~(\ref{eq:mudcap}) 
uniquely suited to study the axial 2-body currents in the 2-N system. 

\begin{figure}[hbt] 
\vspace{-1.cm}  
\begin{center}
\resizebox*{1.\textwidth}{0.5\textheight}{\includegraphics{dp.pdf}} 
\vspace{-1.6cm}
\caption{\label{dp}  $\mu d$ capture Dalitz plot as function of neutron energy. Diagonal lines indicate
constant neutrino momentum $p_\nu$ (MeV/c). Interesting kinematic regions include: 
final state interaction ; quasifree ; $p_\nu \ge 90 MeV/c$,
 where pionless EFT applies; small  $p_\nu$, where
MECs dominate over impulse approximation.}
\end{center}
\vspace{-.4cm}
\end{figure} 

\begin{figure}[hbt] 
\vspace{-0.cm}  
\begin{center}
\resizebox*{.6\textwidth}{0.4\textheight}{\includegraphics{deut_exp.pdf}} 
\vspace{-.6cm}
\caption{\label{f:deut_exp} }
\end{center}
\vspace{-0.cm} 
\end{figure}
Muon capture on the deuteron is
successfully described by two frameworks,
the standard nuclear physics  approach (SNPA)
and by effective field theory (EFT) calculations. 
The most sophisticated SNPA calculation were performed around 
1990~\cite{Tatara:1990eb,Adam:1990kf, Doi:1989kv}. Thereafter the concept of
effective field theories in the form of chiral perturbation theory ($\chi$PT) was
expanded to the 2N system. The latest calculation were performed in hybrid EFT~\cite{Ando:2001es}
and most recently in pion-less EFT~\cite{Chen:2005ak} ($\not{\pi}$EFT). Fig.~\ref{f:deut_exp} summarizes the
theoretical and experimental results.


Current calculations agree that the one body (1B) operators are very well defined. The
challenge lies in the short range part of the axial two body current (2B). In the meson exchange (MEC)
picture it is dominated by the $\pi N N^*$ isobar current, which is not constraint
by general symmetry principles. The systematic expansion of $\chi$PT demonstrated
that exactly the same combinations of low energy constants (LECs) appear in the two
body reactions $p+p$ fusion, $\nu+d$ scattering and $\mu+d$ capture. 
The hybrid EFT used tritium beta decay to constrain the unknown LEC. The $\not{\pi}$EF treats
this LEC called $L_{1A}$ as an unknown parameter and parametrizes the capture rate as
\begin{equation}
 \Lambda_D = a + b~ L_{1A}
\end{equation}
where a and b depend on the $E_{nn}$ Dalitz plot cut. E.g. for $E_{nn}=5\; MeV$, a=239.2\is and 
b=3.3\is$fm^{-3}$. Both calculations
agree if $L_{1A}= 5.6~fm^3$ is used~\cite{Chen:2005ak}  . The hybrid EFT calculation estimates an 
uncertainty 1\%, resulting from
small dependence on cutoff parameter, tritium beta decay rate, higher MEC contributions and
a conservative estimate of the $L\ge1$ partial waves. It also notes that radiative
corrections still need to be calculated. The $\not{\pi}$EF paper concludes that its 
uncertainty of 2-3\% is dominated by N$^3$LO contribution, not yet calculated.

Mention differential oservables. In particular spin correlation (asymmetry) potentially accessible
ofr the first time in muon capture on muonic hydrogen isotopes.

\subsection{Experiment}
The early counter experiments were based on the observation of capture neutrons. 
While a precise measurement of the 
absolute neutron emission rate is difficult even for 5.2 MeV neutrons resulting
from $\mu$p capture, it is even harder for the continuous spectrum of neutrons emitted in 
$\mu$d capture which is peaked at 1.5 MeV. Moreover, numerous 2.45 MeV neutrons are produced
by muon catalyzed dd fusion, representing a significant background. The interpretation
of the experiments requires an accurate knowledge of d$\mu$ hyperfine population at the
moment of capture, because the V-A structure of weak interactions suppresses capture from
the quartet relative to the doublet state. The first generation experiments\cite{Wang:1965, Bertin:1974sr} tried to 
reduce the background from dd fusion, by using hydrogen targets with small deuterium concentration.
Because of the fast p$\mu$ to d$\mu$ transfer rate, such a target acts as an effective
hydrogen target. The price to pay for such an approach is that at high densities capture
occurs from a molecular state and the background from \MHE\ build-up is significant. For lower
densities, on the other hand, the d$\mu$ hyperfine population was essentially unknown at that
time and had to be conjectured as being pure doublet.

\begin{table}[htb]
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline 
 year & $\phi(\%)$ & $c_D (\%)$  &T (K)& detection & statistics & \Rd (s$^{-1}$)& comment \cr
\hline
 1965 & 100        &  0.32         &20&  neutron  &  615       &  365$\pm$96      &  dominant \MHE   \cr
\hline
 1973 & 0.76        &  5       &300&  neutron  &  6295       &  445$\pm$60   & corrected to  
$\approx$ 1335 $\pm$ 180~$^{*)}$ \cr
\hline
 1986 & 100         &  100        &20&  electron  &  5 10$^8$    &  470$\pm$29   &    \cr
\hline
 1989 & 4          &  100         &45&  neutron  &  $\approx$ 2000   &  409$\pm$40   &   \cr
\hline
\end{tabular}
\caption{Counter experiment on $\mu +d $ capture. Density $\phi$ normalized to $LH_2$ density. Experiments performed in D+H mixtures, with $c_D$ given in column 3.  $^{*)}$ Original Result has to be scaled up, because experiment
corresponds to mostly statistical, not doublet d$\mu$ hyperfine population. }
\end{center}
\vspace{-.5cm}
\end{table}


The situation changed with the discovery~\cite{Kammel:1984vu} of a strong dependent temperature hyperfine
effect in resonant dd$\mu$ formation, which made the d$\mu$ hyperfine population directly experimentally
accessible. This and subsequent experimental and theoretical work proved that the conditions
in experiment~\cite{Bertin:1974sr} were statistical, so the observed experimental rates should be scaled
by a factor of 3 to be converted into \Rd, according to the statistical weight of the doublet
state. The resulting contradictory situation stimulated a new generation of experiments based on 
pure deuterium targets. 


One innovation~\cite{Bardin:1986}
 was the detection of electrons with a liquid target at Saclay, which avoided neutron
detection and background from dd fusion. 
Lifetimes of both $\mu^{-}$ and $\mu^{+}$ were measured with
an accuracy of a few times 10$^{-5}$.
The muon lifetime measurement started 1~$\mus$ after 
the beam burst, after muons stopped in wall materials were already captured.
The final rate included corrections for protium ($c_P=0.13\%-0.18 \%$), $\mu ^{3}$He capture $\delta \Lambda=(60\pm16)~s^{-1}$
as well as instrumental effects.

The Vienna PSI experiment~\cite{Cargnelli:1989} on the other hand used neutron detection, but reduced the 
gas density and temperature to suppress fusion neutrons and performed supplemental analyses with high neutron
threshold above the 2.5 MeV fusion neutrons. In the low density target the stopping fraction of muons in
$D_2$ was $(75.7\pm1.7)\%$. The physics background, consisting of carbon stops, diffusion,
photo neutrons and fusion neutrons, exceeded the physics signal by a factor of 1.4 and uncertainties 
in its subtraction dominated the error of the final result.   

The current  overall experimental situation 
on $\Lambda_{D}$ (see Fig.\ref{f:deut_exp}) is quite unsatisfactory. The best two measurements 
were performed almost two decades ago. They have uncertainties of 10-15\% and are only marginally consistent,
with the more accurate experiment deviating from theory by 2.4 $\sigma$. 



\subsection{Status of Basic Muon Capture Reactions}

Discuss mu+p, mu+d and mu+3He, including the recent rad corr update~\cite{Czarnecki:2007th}.
Can we trust the 0.5\% precision of calculation~\cite{Marcucci:2000xy}.


\subsection{$L_{1A}$ extraction}
The current theoretical uncertainty for $\Lambda_D$ ranges from 1-3\%. Assuming
an  experimental determination of  $\Lambda_D$ with 1\% precision $L_{1A}$ would be determined
as
\begin{equation}
\delta L_{1A} \sim
\frac{a}{b} \sqrt{\frac{\delta \Lambda_D^{th}}{\Lambda_D^{th}}^2  +
\frac{\delta \Lambda_D^{exp}}{\Lambda_D^{exp}}^2
}
\end{equation} 
which gives

\begin{center}
\begin{tabular}{c c}
$ \frac{\delta \Lambda_D^{th}}{\Lambda_D^{th}} (\%)$ & $\delta L_{1A} (fm^{-3})$\\
0  & 0.71  \\ 
1  & 1.0   \\
2  & 1.2   \\
3  & 1.4   \\
\end{tabular}
\end{center}


Given this impressive precision claimed we critically discuss uncertainties due to additional physics
input.  The sensitivity to $g_P$ is $\frac{\delta\Lambda_D}{\Lambda_D}/\frac{\delta g_P}{g_P}=0.2$. Thus 
final MuCap result for $g_P$ at the 1\% level, is a prerequisite for determining L$_{1A}$ from muon
capture. The $g_P$ uncertainty will contribute $\frac{\delta\Lambda}{\Lambda}=xx\% $. NEEDs discussion
on uncertainty reduction if capture rates are compared, theory also.
The dependency on the neutron scattering length $a_{nn}$ would
only lead to $\frac{\delta\Lambda}{\Lambda}= 0.9\% $, if the currently accepted value of 
$a_{nn}= -18.6 \pm 0.4~fm$ is being used. This value is derived exclusively from the 
$\pi d \rightarrow n+ n + \nu$ reaction and does
not take the deviating results for n+d break-up into account~\cite{Machleidt:2001rw,GonzalezTrotter:2006wz}.





==> Reference.tex <==
\makeatletter
\newcommand{\bibname}{References}
\renewenvironment{thebibliography}[1]
     {\section{\bibname}%
      \list{\@biblabel{\@arabic\c@enumiv}}%
           {\settowidth\labelwidth{\@biblabel{#1}}%
            \leftmargin\labelwidth
            \advance\leftmargin\labelsep
            \@openbib@code
            \usecounter{enumiv}%
            \let\p@enumiv\@empty
            \renewcommand\theenumiv{\@arabic\c@enumiv}}%
      \sloppy
      \clubpenalty4000
      \@clubpenalty \clubpenalty
      \widowpenalty4000%
      \sfcode`\.\@m}
\makeatother
%\section{References}

\bibliography{prop07}{}
\bibliographystyle{unsrt}
%\addcontentsline{toc}{section}{\protect\numberline{}References}

%\input{references.tex}


==> Safety.tex <==
\section*{Safety Sheet}


The third page should consist of the declaration sheet for hazardous samples/equipment ( PDF, Word) . This does not replace a detailed description of safety questions  in the full text of the proposal.


Safety Procedure for R-Experiments

The purpose of this document is to guide applicants for R-Experiments  (experiments at the 590 MeV Ring Cyclotron) through the different safety regulations and procedures applicable at PSI concerning hazardous equipment and sample material.

General

If you intend to work with hazardous equipment and material, the first persons to be contacted are the Safety Officers of your home institution. They must inform you about all potential risks involved. They will also inform you about the regulations applicable in your country.

The Responsibility for Hazardous Equipment and Sample Material at PSI lies with the Experiment Spokespersons.
In case of a test experiment the coordinator of these tests is responsable for safety. The PSI safety procedures listed below are obligatory for them.

The Safety Officers of PSI are available to help you fulfilling the necessary regulations applicable to PSI. You must contact them well in advance.


Safety of your equipment.

In designing your experiment or in case you change your approved experimental set-up, you should proceed as follows:

   1. Contact the Coordinator for R-Experiments  to discuss the instrument's design or planned modifications.
   2. Use the Declaration Sheet for Hazardous Sample/Target Material and Experimental Equipment (PDF, Word) of the Safety Committee PSI West to characterize the hazards of your equipment. Add the Declaration sheet to your proposal. You are in addition requested to describe the safety risks of your experiment in the text of your proposal.
   3. When the design of the equipment is finalized, contact the appropriate members of the Safety Committee. The Safety Officers will discuss with you the necessary safety precautions and authorisations for your equipment.
   4. Before installing new or modified equipment at PSI for the first time, contact the Safety Committee again to allow inspection of your equipment.


Hazardous sample material.

When you intend to investigate hazardous sample material (radioactive, toxic, flammable, etc.) on your experiment, proceed as follows:

   1. Use the Declaration Sheet for Hazardous Sample/Target Material and Experimental Equipment (PDF, Word) of the Safety Committee PSI West to characterize the hazards of your sample.
   2. Contact the appropriate members of the Safety Committee well in advance. The Safety Officers will discuss with you the necessary safety precautions, authorisations and handling procedures.

\newpage
